Riddim: A Rhythm Analysis and Decomposition Tool Based On Independent Subspace Analysis

The goal of this thesis was to implement a tool that, given a digital audio input, can extract and represent rhythm and musical time. The purpose of the tool is to help develop better models of rhythm for real-time computer based performance and composition. This analysis tool, Riddim, uses Independent Subspace Analysis (ISA) and a robust onset detection scheme to separate and detect salient rhythmic and timing information from different sonic sources within the input. This information is then represented in a format that can be used by a variety of algorithms that interpret timing information to infer rhythmic and musical structure. A secondary objective of this work is a "proof of concept" as a non-real-time rhythm analysis system based on ISA. This is a necessary step since ultimately it is desirable to incorporate this functionality in a real-time plug-in for live performance and improvisation.

==> abstract.tex <==

The goal of this thesis was to implement a tool that, given
a digital audio input, can extract and represent rhythm and musical 
time. The purpose of the tool is to help develop better models of 
rhythm for real-time computer based performance and composition. 
This analysis tool, {\sl Riddim}, uses Independent Subspace Analysis 
(ISA) and a robust onset detection scheme to separate and detect 
salient rhythmic and timing information from different sonic sources 
within the input. This information is then represented in a format 
that can be used by a variety of algorithms that interpret timing 
information to infer rhythmic and musical structure. 
A secondary objective of this work is a ``proof of concept'' as a
non-real-time rhythm analysis system based on ISA.  This is a necessary 
step since ultimately it is desirable to incorporate this functionality in a
real-time plug-in for live performance and improvisation.

==> acknowledgements.tex <==
I would like to thank Roger Dannenberg for introducing me to this
field and writing me a recommendation for Dartmouth. Arigato gozaimasu
to my teachers Jon Appleton, Eric Lyon, Charles Dodge 
and Larry Polanksy for providing the opportunity to attend Dartmouth 
and the nurturing environment to develop and produce this work.  

Ridiculous amounts of thanks to Hany Farid for signing on to be an
advisor and tolerating random emails for help throughout the year.

Major muchas gracias to Ray Guillette for moral support, advice and 
assistance with the design of {\it Riddim}'s Graphical User
Interface. Cheers to Michael Casey for providing MATLAB demos, 
suggestions and feedback that ultimately enabled this work. Thanks to 
John Puterbaugh for technical advice and book suggestions 
like ``Conceptual Spaces''.

Vielen Dank to Barbara Tillmann and D{\^ e}kuji to Petr Janata for 
reviewing the final document on such short notice and giving many 
useful comments.

Tusen takk to the nordic nightmare for offering suggestions, papers to
read and numerous insights on rhythm. Mahalo nui loa to Moki for 
reviewing the kosherness of my diagrams and generally adding
value. And grazie mille to Dee for making the world a safer place 
for everybody!!



==> chapter6.tex <==
\chapter{Conclusions and Avenues of Further Study}
\vspace{7mm}

\begin{quote}
  {\sl ``I conclude that musical notes and rhythms were first acquired
    by the male and femail progenitors of mankind for the sake of
    charming the opposite sex.''} --- Charles Darwin
\end{quote}




==> dedication.tex <==

\begin{quote}
{This work is dedicated to my parents and to the 
loving memory of my grandfathers Samuel Moniruvwe Orife 
and William Kendall Ford.}
\end{quote}





==> preface.tex <==
This is the preface ....

